Is your vote truly secret? Ballot Secrecy iff Ballot Independence: Proving necessary conditions and analysing case studies

We formalise definitions of ballot secrecy and ballot independence by Smyth, JCS'21 as indistinguishability games in the computational model of security. These definitions improve upon Smyth, draft '21 to consider a wider class of voting systems. Both Smyth, JCS'21 and Smyth, draft '21 improve on earlier works by considering a more realistic adversary model wherein they have access to the ballot collection. We prove that ballot secrecy implies ballot independence. We say ballot independence holds if a system has non-malleable ballots. We construct games for ballot secrecy and non-malleability and show that voting schemes with malleable ballots do not preserve ballot secrecy. We demonstrate that Helios does not satisfy our definition of ballot secrecy. Furthermore, the Python framework we constructed for our case study shows that if an attack exists against non-malleability, this attack can be used to break ballot secrecy.

==> Results/old.tex <==
\begin{proof}
Suppose $\Gamma$ does not satisfy {\BS}, then there exists a probabilistic polynomial-time adversary $\mathcal{A}$, such that for all candidates in the set of candidates $V$ and all negligible functions {\fontfamily{lmss}\selectfont negl}, there exists a security parameter $k$ such that {\fontfamily{lmss}\selectfont Succ(Ballot Secrecy($\Gamma$, $\mathcal{A}$, $V$, $k$) $>$ $\frac{1}{2} + $ {\fontfamily{lmss}\selectfont negl}($k$)}. We construct an adversary $\mathcal{B}$ against {\NM} \ from $\mathcal{A}$. 

We begin by constructing two games that combined, represent {\BS}, under the assumption that {\BS} satisfies additivity: {\BSA} and {\BSC}. 

{\BSA} as defined below, is equivalent to {\BS} except the bulletin board only contains ballots constructed by the adversary. Line 1 is equivalent to Line 1 in {\BS}. A set is initialised to keep track of the challenge ballots. (Line 2) The adversary decides which vote the ballot that they construct will contain (Line 3), then constructs the ballot (Line 4). A bulletin board is constructed exclusively from the adversarial ballots (Line 5). Line 6 and 7 are equivalent to the ones in {\BS}. To win the game, the adversary in {\BSA} must return the value of the coin (bit $\beta$) (this is trivial as the adversary picks the coins), the bulletin board must satisfy the balanced condition and only contain adversary constructed ballots. Adversary ballots are denoted as $\mathfrak{b}$ whereas challenge ballots are denoted as $b$.

\LinesNumbered
\begin{algorithm*}[H]

\SetKw{Return}{return}

$\mathnormal{pk, sk} \gets \mathrm{Setup}(k) $\;
$L \gets \emptyset$\;
$\mathnormal{v_\beta}$ $\gets$ $\mathcal{A}(pk, k)$\;
$\mathfrak{b}$ $\gets$ $\mathrm{Vote}(pk, v_\beta, k)$\;
$\mathfrak{bb'}$ $\gets$ $\mathcal{A}(\mathfrak{b})$\;
$\mathnormal{e}$ $\gets$ $\mathrm{Partial-Tally}(sk, \mathfrak{bb'}, k)$\;

$\mathnormal{g}$ $\gets$ $\mathcal{A}(\mathfrak{bb'}, e)$\;

\BlankLine
\Return $g = \beta$ $\wedge$ $balanced(\mathfrak{bb'}, V, L) \wedge v_0, v_1 \in V$\;

\caption{BS-A($\Gamma$, $\mathcal{A}$, $V$, $k$)}
\end{algorithm*}

\label{algorithm:posit}
\textit{We say} $\Gamma$ \textit{satisfies} {\fontfamily{lmss}\selectfont BS-A} \textit{if for all probabilistic polynomial time adversaries} $\mathcal{A}$ \textit{and all sets of candidates} $V$, \textit{there exists a negligible function} {\fontfamily{lmss}\selectfont negl}, \textit{such that for all security parameters} $k$, \textit{we have:}\\
{\fontfamily{lmss}\selectfont Succ(BS-A($\Gamma$, $\mathcal{A}$, $V$, $k$) $\leq$ $ 1 -$ {\fontfamily{lmss}\selectfont negl}($k$)}.

Subsequently we present game {\BSC}, which is equivalent to {\BS} except for the bulletin board, which only contains challenge ballots. Lines 1, 2 and 3 are equivalent to the ones in {\BS}. In line 4, the adversary computed the bulletin board exclusively from the calls to the left-right oracle, which returns the challenge ballots. This oracle is defined as per {\BS}. Lines 5 and 6 are equivalent to lines 4 and 5 respectively in {\BS}. To win the game, the adversary must guess the coin (bit $\beta$), ensure that the bulletin board satisfies the balanced condition and that it only contains challenge ballots. (Line 7).

\LinesNumbered
\begin{algorithm*}[H]

\SetKw{Return}{return}

$\mathnormal{pk, sk} \gets \mathrm{Setup}(k) $\;
$\mathnormal{\beta}$ $\gets$ $\mathnormal{_R\{0, 1\}}$\;
$L \gets \emptyset$\;
$\mathfrak{bb''}$ $\gets$ $\mathcal{A^O}(pk, k)$\;
$\mathnormal{e}$ $\gets$ $\mathrm{Partial-Tally}(sk, \mathfrak{bb''}, k)$\;
$\mathnormal{g}$ $\gets$ $\mathcal{A}(\mathfrak{bb''}, e)$\;

\BlankLine
\Return $g = \beta$ $\wedge$ $balanced(\mathfrak{bb''}, V, L) \ \wedge $ \ $v_0, v_1 \in V$\;

\caption{BS-C($\Gamma$, $\mathcal{A}$, $V$, $k$)}
\end{algorithm*}

\label{algorithm:posit}
\textit{We say} $\Gamma$ \textit{satisfies} {\fontfamily{lmss}\selectfont BS-C} \textit{if for all probabilistic polynomial time adversaries} $\mathcal{A}$ \textit{and all sets of candidates} $V$, \textit{there exists a negligible function} {\fontfamily{lmss}\selectfont negl}, \textit{such that for all security parameters} $k$, \textit{we have:}\\
{\fontfamily{lmss}\selectfont Succ(BS-C($\Gamma$, $\mathcal{A}$, $V$, $k$) $\leq$ $\frac{1}{2} + $ {\fontfamily{lmss}\selectfont negl}($k$)}

Assuming that {\BS} satisfies additivity, it can be said that the bulletin board of {\BS} is the sum of the bulletin board of {\BSA} and the bulletin board of {\BSC}. 
Because the {\BS} bulletin board is constructed with both adversarial and challenge ballots, both {\BSA} and {\BSC} are necessary for {\BS}, as we cannot know in advance the adversary's strategy to win {\BS}.

Proof sketch:
We show that given an adversary A that wins {\BSA} exists, we can construct an adversary B to win NM.
We show that given an adversary A that wins {\BSC} exists, we can construct an adversary B to win NM.
However, this does not suffice to demonstrate NM => BS. We must have an adversary that wins BOTH {\BSA} and {\BSC}. To achieve this, we can simulate {\BS} as a series of {\BSA} and {\BSC} games where the order of them and how many of them there are is arbitrary, because there are no conditions on how many adversarial vs challenge ballots must be in {\BS}'s bulletin board and in what order they must appear. 

Proof of Theorem [{\BS} \ $\Rightarrow$ {\NM}].\\

Suppose $\Gamma$ does not satisfy {\BSA}, there exists a probabilistic polynomial-time adversary $\mathcal{A}$, such that for all candidates in set of candidates $V$ and all negligible functions {\fontfamily{lmss}\selectfont negl}, there exists a security parameter $k$ such that {\fontfamily{lmss}\selectfont Succ({\BSA}($\Gamma$, $\mathcal{A}$, $V$, $k$)) $>$ $\frac{1}{2} + $ {\fontfamily{lmss}\selectfont negl}($k$)}. We construct an adversary $\mathcal{B}$ against {\NM} \ from $\mathcal{A}$. 
\begin{itemize}
    \item $\mathcal{B}(pk, k)$ computes $v_\beta \gets \mathcal{A}(pk, k)$.
    \item $\mathcal{B}(b)$ computes $\mathfrak{bb'} \gets \mathcal{A}(b)$. 
   \item $\mathcal{B}(\mathfrak{v})$ computes $e \gets \mathrm{Partial-Tally}(sk, \mathfrak{bb'},k)$; $g \gets \mathcal{A}(\mathfrak{bb'}, e)$ and returns $g = \beta \ \wedge \\ balanced(\mathfrak{bb'}, V, L) \ \wedge v_0, v_1 \in V.$

\end{itemize}
Adversary $\mathcal{B}$ wins {\NM} because $\mathfrak{bb'}$ is balanced and contains only adversary ballots, so {\NM}'s challenge ballot will not be in the bulletin board. As such, $\mathcal{B}$ satisfies all the criteria to win {\NM} from the adversary $\mathcal{A}$ of {\BSA}, concluding our proof.

Suppose $\Gamma$ does not satisfy {\BSC}, there exists a probabilistic polynomial-time adversary $\mathcal{A}$, such that for all candidates in set of candidates $V$ and all negligible functions {\fontfamily{lmss}\selectfont negl}, there exists a security parameter $k$ such that {\fontfamily{lmss}\selectfont Succ({\BSC}($\Gamma$, $\mathcal{A}$, $V$, $k$)) $>$ $1 - $ {\fontfamily{lmss}\selectfont negl}($k$)}. We construct an adversary $\mathcal{B}$ against {\NM} \ from $\mathcal{A}$. 
\begin{itemize}
    \item $\mathcal{B}(pk, k)$ computes $\mathfrak{bb''} \gets \mathcal{A^O}(pk, k)$;
    \item $\mathcal{B}(b)$ does nothing.
   \item $\mathcal{B}(\mathfrak{v})$ computes $e \gets \mathrm{Partial-Tally}(sk, \mathfrak{bb''},k)$; $g \gets \mathcal{A}(\mathfrak{bb''}, e)$ and returns $g = \beta \ \wedge \\ \ balanced(\mathfrak{bb''}, V, L) \ \wedge v_0, v_1 \in V.$

\end{itemize}
Adversary $\mathcal{B}$ wins {\NM} because $\mathfrak{bb''}$, despite only containing challenge ballots, does not contain {\NM}'s challenge ballot. This is because $\mathfrak{bb''}$ is computed before the second adversary call in {\NM}, when the adversary receives the challenge ballot $b$, so $\mathcal{A}$ cannot have added $b$ to $\mathfrak{bb''}$ before this ballot was computed and given to the adversary. After this, $\mathcal{B}$ cannot add $b$ to $\mathfrak{bb''}$, otherwise it will lose the game. The second adversary call does not need to compute anything, as the bulletin board was already constructed from the previous adversary call. As such, $\mathcal{B}$ satisfies all the criteria to win {\NM} from the adversary $\mathcal{A}$ of {\BSA}, concluding our proof.

Finally we must show that {\BS} can be played as a series of {\BSA} and {\BSC} games. 
(How do I do that? It seems intuitive?)

Because we have demonstrated that:
\begin{itemize}
    \item Having an adversary that wins {\BS} means an adversary exists that can win an arbitrary combination of {\BSA} and {\BSC} games.
    \item From a winning adversary against {\BSA} we can construct a winning adversary against {\NM}.
    \item From a winning adversary against {\BSC} we can construct a winning adversary against {\NM}.
\end{itemize}

We can combine the adversaries in an arbitrarily long series of {\BSA} and {\BSC} games in any order to simulate {\BS}, and since we know we can construct a winning adversary against {\NM} from each, we can demonstrate that by having a winning adversary against {\BS}, we can construct a winning adversary against {\NM}, thus concluding our proof.
\end{proof}

*define additivity: tallying bb is the same as tallying first the bb' that contains only adversary ballots and then adding this to bb'' that contains only challenge ballots.
